Simultaneous temperature estimation and nonuniformity correction from multiple frames

IR cameras are widely used for temperature measurements in various applications, including agriculture, medicine, and security. Low-cost IR cameras have the immense potential to replace expensive radiometric cameras in these applications; however, low-cost microbolometer-based IR cameras are prone to spatially variant nonuniformity and to drift in temperature measurements, which limit their usability in practical scenarios. To address these limitations, we propose a novel approach for simultaneous temperature estimation and nonuniformity correction (NUC) from multiple frames captured by low-cost microbolometer-based IR cameras. We leverage the camera's physical image-acquisition model and incorporate it into a deep-learning architecture termed kernel prediction network (KPN), which enables us to combine multiple frames despite imperfect registration between them. We also propose a novel offset block that incorporates the ambient temperature into the model and enables us to estimate the offset of the camera, which is a key factor in temperature estimation. Our findings demonstrate that the number of frames has a significant impact on the accuracy of the temperature estimation and NUC. Moreover, introduction of the offset block results in significantly improved performance compared to vanilla KPN. The method was tested on real data collected by a low-cost IR camera mounted on an unmanned aerial vehicle, showing only a small average error of $0.27-0.54^\circ C$ relative to costly scientific-grade radiometric cameras. Our method provides an accurate and efficient solution for simultaneous temperature estimation and NUC, which has important implications for a wide range of practical applications.

==> results/_real_data_registration_process.tex <==
\noindent Registration transforms all frames to the same coordinate system, such that an object has equal coordinates across all frames.
Contrary to previous works, we do not make assumptions on the reference frame. To maximize the redundant information between frames, a plane $\mathcal{I}$\ that maximizes the overlap between frames must be found. Notice that finding the ideal $\mathcal{I}$ is infeasible, because it requires solving an expensive optimization problem. Instead, $\mathcal{I}$ is approximated as the frame with the maximal overlap to all other frames.

Kernels have a finite support and limited receptive field, so the frames are registered before entering the network.
We used the classic feature extraction algorithm SIFT by Lowe~\cite{sift}. 
SIFT identifies distinctive keypoints in a frame. A descriptor vector of 128 values is extracted for each keypoint, based on the directional gradients in the area surrounding the keypoint.

To match keypoints between frames, we used mutual nearest neighbor (MNN) distance with Euclidean distance to measure the similarity between vectors. MMN means finding pairs of vectors in a set that minimizes the Euclidean distance for each other. Two vectors are MNN if they have the minimal distance towards each other in their sets.

The overlap between frames was determined by counting the positive pixels in the overlapping masks. That is, after performing a pixel-wise AND operator on all the masks created by the homography of each frame.

The registration process differs between the training and validation (inference).
\subsubsection{Training}
% A number of homographies were randomly sampled for each frame, creating different views of the same frame. The inverse homographies were used to register all the views towards the original frame, which is de-facto $\mathcal{I}$. 
% Random deviations of up to $\pm2$ pixels were added to the inverse homographies to simulate imperfect registration.
% These registered views were fed into the network.

\subsubsection{Validation and any other inference}
Homographies were randomly sampled, but the inverses of the homographies were discarded. Instead, $\mathcal{I}$ was approximated for each burst by SIFT and MNN as described above. 
All frames in the burst were registered to the approximated $\mathcal{I}$.
All results presented in this work were obtained using this method.
The same homographies were used for validation throughout all experiments and ablations.

% The sampled homographies either create a random walk from one side of the temperature map to the other side, or a hover above a random point.

% The registration method was implemented with the package Kornia~v0.67.
